Optimal vaccination in a stochastic epidemic model of two non-interacting populations

Developing robust, quantitative methods to optimize resource allocations in response to epidemics has the potential to save lives and minimize health care costs. In this paper, we develop and apply a computationally efficient algorithm that enables us to calculate the complete probability distribution for the final epidemic size in a stochastic Susceptible-Infected-Recovered (SIR) model. Based on these results, we determine the optimal allocations of a limited quantity of vaccine between two non-interacting populations. We compare the stochastic solution to results obtained for the traditional, deterministic SIR model. For intermediate quantities of vaccine, the deterministic model is a poor estimate of the optimal strategy for the more realistic, stochastic case.

==> mybib.tex <==
@article{medlock, 
author = "Jan Medlock and Alison P. Galvani",
title = "Optimizing Influenza Vaccine Distribution", 
journal = "Science", 
year = "2009", 
volume="325",
number="5948",
pages="1705-1708",
} 

@article{knipl, 
author = "Diána H. Knipl and Gergely Rost",
title = "Modelling the strategies for age specific vaccination scheduling during influenza pandemic outbreaks", 
journal = "Mathematical Biosciences and Engineering", 
year = "2011", 
volume="8",
number="5948",
pages="123-139",
} 

@article{kermack, 
author = "W. O. Kermack and A. G. McKendricki",
title = "A contribution to the Mathematical Theory of Epidemics", 
journal = "Proc. R. Soc. Lond. A", 
year = "1927", 
volume="115",
number="772",
pages="700-721",
} 

@article{gaff, 
author = "H. Gaff and E. Schaefer",
title = "A contribution to the Mathematical Theory of Epidemics", 
journal = "Mathematical Biosciences and Engineering", 
year = "2009", 
volume="6",
number="",
pages="469-492",
} 

@article{klepac, 
author = "Petra Klepac and Ramanan Laxminarayan and Bryan T. Grenfell",
title = "Synthesizing epidemiological and economic optima for control of immunizing infections", 
journal = "Proc Natl Acad Sci U S A.", 
year = "1927", 
volume="108",
number="34",
pages="14366-14370",
} 

@article{tildesley, 
author = "Michael J. Tildesley and Nicholas J. Savill and Darren J. Shaw and Rob Deardon and Stephen P. Brooks and Mark E. J. Woolhouse and Bryan T. Grenfell and Matt J. Keeling",
title = "Synthesizing epidemiological and economic optima for control of immunizing infections", 
journal = "Nature", 
year = "2006", 
volume="440",
number="7080",
pages="83-86",
} 

@article{keeling1, 
author = "Matt J. Keeling and Mark E. J. Woolhouse and Darren J. Shaw and Louise Matthews and Margo Chase-Topping and Dan T. Haydon and Stephen J. Cornell and Jens Kappey and John Wilesmith and Bryan T. Grenfell1l",
title = "Dynamics of the 2001 UK Foot and Mouth Epidemic: Stochastic Dispersal in a Heterogeneous Landscape", 
journal = "Science", 
year = "2001", 
volume="294",
number="5543",
pages="813-817",
} 

@article{groenendaal, 
author = "Huybert Groenendaal and Mirjam Nielena and Alien W. Jalvingha and Suzan H. Horsta and David T. Galliganb and Jan Willem Hesselink",
title = "A simulation of Johne's disease controls", 
journal = "Prev. Vet. Med.", 
year = "2002", 
volume="54",
number="",
pages="225-245",
} 

@article{grenfell, 
author = "Bryan T. Grenfel and Ottar N. Bjornstad and J. Kappey",
title = "Travelling waves and spatial hierarchies in measles epidemics", 
journal = "Science", 
year = "2001", 
volume="414",
number="",
pages="716-723",
} 

@article{hufnagel, 
author = "L. Hufnagel and D. Brockmann and T. Geisel",
title = "Forecast and control of epidemics in a globalized world", 
journal = "Proc Natl Acad Sci U S A", 
year = "1927", 
volume="101",
number="42",
pages="15124–15129",
} 

@article{keeling2, 
author = "Matt J. Keeling and Andrew Shattock",
title = "Optimal but unequitable prophylactic distribution of vaccine", 
journal = "Epidemics", 
year = "2012", 
volume="4",
number="2",
pages="78-85",
} 

@article{gordillo, 
author = "Luis F. Gordillo and Stephen A. Marion and Anders Martin-Löfc and Priscilla E. Greenwood",
title = "Bimodal epidemic size distributions for near-critical SIR with vaccination", 
journal = "Bulletin of Mathematical Biology", 
year = "2008", 
volume="70",
number="",
pages="589-602",
} 

@article{jenkinson, 
author = "Garrett Jenkinson and John Goutsias",
title = "Numerical Integration of the Master Equation in Some Models of Stochastic Epidemiology", 
journal = "PLoS ONE", 
year = "2012", 
volume="7",
number="5",
pages="e36160",
} 

@article{petrovic, 
author = "Nada Petrovic and David L. Alderson and Jean M. Carlson",
title = "Dynamic Resource Allocation in Disaster Response: Tradeoffs in Wildfire Suppression", 
journal = "PLoS ONE", 
year = "2012", 
volume="7",
number="",
pages="e33285",
} 

@article{keeling3, 
author = "MJ Keeling and JV Ross",
title = "On methods for studying stochastic disease dynamics", 
journal = "J R Soc Interface", 
year = "2008", 
volume="5",
number="",
pages="171-181",
} 

@article{munsky, 
author = "B Munsky and M Khammash",
title = "The finite projection algorithm for the solution of the chemical master equation", 
journal = "J Chem Phys", 
year = "2006", 
volume="124",
number="",
pages="044104",
} 

@article{jong, 
author = "Mart C.M. De Jong and Annemarie Bouma",
title = "Herd immunity after vaccination: how to quantify it and how to use it to halt disease", 
journal = "Vaccine", 
year = "2001", 
volume="19",
number="",
pages="2722-2728",
} 

@article{anderson, 
author = "M.R. Anderson and R.M. May",
title = "Directly transmitted infections diseases: control by vaccination?", 
journal = "Science", 
year = "1982", 
volume="215",
number="4536",
pages="1053–1060",
} 

@article{leroux, 
author = "Isabel Leroux-Roels and Geert Leroux-Roels",
title = "Current status and progress of prepandemic and pandemic influenza vaccine development", 
journal = "Expert Review of Vaccines", 
year = "2009", 
volume="8",
number="4",
pages="401-423",
} 

@article{wu, 
author = "Joseph T. Wu and Steven Riley and Gabriel M. Leung",
title = "Spatial considerations for the allocation of pre-pandemic inﬂuenza vaccination in the United States", 
journal = "Proc. R. Soc. B", 
year = "2007", 
volume="274",
number="1627",
pages="2811-2817",
} 
